Webly Supervised Concept Expansion for General Purpose Vision Models

General Purpose Vision (GPV) systems are models that are designed to solve a wide array of visual tasks without requiring architectural changes. Today, GPVs primarily learn both skills and concepts from large fully supervised datasets. Scaling GPVs to tens of thousands of concepts by acquiring data to learn each concept for every skill quickly becomes prohibitive. This work presents an effective and inexpensive alternative: learn skills from supervised datasets, learn concepts from web image search, and leverage a key characteristic of GPVs: the ability to transfer visual knowledge across skills. We use a dataset of 1M+ images spanning 10k+ visual concepts to demonstrate webly-supervised concept expansion for two existing GPVs (GPV-1 and VL-T5) on 3 benchmarks: 5 COCO-based datasets (80 primary concepts), a newly curated series of 5 datasets based on the OpenImages and VisualGenome repositories (~500 concepts), and the Web-derived dataset (10k+ concepts). We also propose a new architecture, GPV-2 that supports a variety of tasks -- from vision tasks like classification and localization to vision+language tasks like QA and captioning, to more niche ones like human-object interaction detection. GPV-2 benefits hugely from web data and outperforms GPV-1 and VL-T5 across these benchmarks. Our data, code, and web demo are available at https://prior.allenai.org/projects/gpv2.

==> figs/web_concepts.tex <==
\begin{figure}[h]
    \centering
    \includegraphics[trim=2em 2em 0 0, clip, width=\columnwidth]{figs/web_concepts.pdf}
    \caption{\textbf{Diversity of concepts in \web} visualized through TSNE~\cite{Maaten2008tsne} plot of Phrase-BERT~\cite{Wang2021PhraseBERT} embeddings of nouns with bubble size indicating frequency (capped at 1000) in \cc, a common large-scale pretraining dataset. Nouns in \web\ cover a wide range of concept groups identified using WordNet and include many which are infrequent or absent from \cc.}
    \label{fig:web_concepts}
\end{figure}

==> sections/10_conclusion.tex <==
\section{Conclusion}
\label{sec:conclusion}


==> tables/skills_io.tex <==
% Please add the following required packages to your document preamble:
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{table}[]
\footnotesize
\centering
\setlength{\tabcolsep}{2.5pt}
\begin{tabular}{l|ccc|cc}
\toprule
\rowcolor[HTML]{FFFFFF} 
\textbf{}                             & \multicolumn{3}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{Inputs}}                                                                                                                                               & \multicolumn{2}{c}{\cellcolor[HTML]{FFFFFF}\textbf{Outputs}}                                             \\
\rowcolor[HTML]{FFFFFF} 
{\color[HTML]{000000} \textbf{Skill}} & {\color[HTML]{000000} Image} & {\color[HTML]{000000} \begin{tabular}[c]{@{}c@{}}Text / Prompt \\ Examples\end{tabular}}                                                               & {\color[HTML]{000000} Bbox}                                   & {\color[HTML]{000000} Text} & {\color[HTML]{000000} \begin{tabular}[c]{@{}c@{}}Bbox with \\ scores\end{tabular}}                                    \\ \midrule
\rowcolor[HTML]{EFEFEF} 
\textit{VQA}                          & Full                         & Question                                                                                                    & -                                                             & Answer                      & \begin{tabular}[c]{@{}c@{}}Attended\\ regions\end{tabular}                                                           \\
\rowcolor[HTML]{FFFFFF} 
\textit{Cap}                          & Full                         & \begin{tabular}[c]{@{}c@{}}Describe the image.\\ Caption this image.\end{tabular}                           & -                                                             & Caption                     & \begin{tabular}[c]{@{}c@{}}Attended\\ regions\end{tabular}                                                           \\
\rowcolor[HTML]{EFEFEF} 
\textit{Loc}                          & Full                         & \begin{tabular}[c]{@{}c@{}}Find {[}OBJECT{]}.\\ Locate instances of \\ {[}OBJECT{]}.\end{tabular} & -                                                             & -                           & \begin{tabular}[c]{@{}c@{}}Localized \\ {[}OBJECT{]}\\ instances\end{tabular} \\
\rowcolor[HTML]{FFFFFF} 
\textit{Cls}                          & Cropped                      & \begin{tabular}[c]{@{}c@{}}What is this thing?\\ What object is this?\end{tabular}                          & -                                                             & Category                    & -                                                                          \\
\rowcolor[HTML]{EFEFEF} 
\textit{CiC}                          & Full                         & \begin{tabular}[c]{@{}c@{}}What is this thing?\\ What object is this?\end{tabular}                          & \begin{tabular}[c]{@{}c@{}}Region to \\ classify\end{tabular} & Category                    & -                                                                          \\ \bottomrule
\end{tabular}
\caption{
\label{tab:skill_io}
\textbf{I/O for the 5 skills in \coco\ and \opensce\ evaluation.}} %\todo{Make into single column}}
\end{table}

==> tables/tab_dce_benchmark.tex <==

\begin{table*}
\setlength{\tabcolsep}{2pt}
\footnotesize
\centering
\resizebox{0.5\textwidth}{!}{
\begin{tabular}{
    lc
    >{\columncolor{Color2}}c>{\columncolor{Color2b}}c>{\columncolor{Color2}}c>{\columncolor{Color2b}}c>{\columncolor{Color2}}c
    }

\toprule
\multicolumn{1}{l}{} & \multicolumn{1}{c}{} 
    & \multicolumn{5}{c}{\cellcolor{Color2}\opensce}  \\

\multicolumn{1}{c}{Model} & \multicolumn{1}{c}{Web data} 
    
    & \cellcolor{Color2}\emph{VQA}  
    & \cellcolor{Color2}\emph{Cap} 
    & \cellcolor{Color2}\emph{Loc}
    & \cellcolor{Color2}\emph{Cls}
    & \cellcolor{Color2}\emph{CiC} \\
    
\midrule
%\textcolor{tabindex}{[a]} \gpvone & no web &  45.3 & 25.8 & 61.9 & 10.1 & - \\
%\textcolor{tabindex}{[b]} $\gpvone^{20}$ & no web & 44.3 & 23.1 & 60.3 & 9.3 & - \\
%\textcolor{tabindex}{[c]} $\gpvone^{20}$ & with web & 45.8 & 28.6 & 61.5 & 20.0 & - \\
%\midrule
%\textcolor{tabindex}{[d]} \vltf & no web & 60.2 & 31.6 & - & 10.9 & - \\
%\textcolor{tabindex}{[e]} \vltf & with web &  59.9 & 45.0 & - & 16.2 & - \\
%\midrule
\textcolor{tabindex}{[a]} \gpvtwo & no web & 60.6 & 65.4 & 74.8 & 36.3 & 43.6 \\
\textcolor{tabindex}{[b]} \gpvtwo & with web & 61.1 & 72.5 & 75.9 & 45.4 & 52.2 \\
\midrule
\textcolor{tabindex}{[c]} ViLT \cite{Kim2021ViLTVT} & - & 65.8 & - & - & - & - \\
\textcolor{tabindex}{[d]}  VinVL+VIVO \cite{Zhang2021VinVLMV} & - & - & 78.0 & - & - & - \\
\textcolor{tabindex}{[e]} UniversalCap (w/ CLIP) \cite{Cornia2021UniversalCL} & - & - & 110.4 & - & - & - \\
\textcolor{tabindex}{[f]} VinVL \cite{Zhang2021VinVLMV} & - & - & - & 70.3 & - & - \\
\textcolor{tabindex}{[g]} SWiN \cite{Liu2021SwinTH}& - & - & - & - & 57.2 & - \\
\bottomrule
\end{tabular}}
\caption{
\label{tab:dce_baselines}
\textbf{Calibrating DCE with Specialized Models.} \todo{Justify gap in performance}
\opensce~Cap only shows out-of-domain results from nocaps due to limited space.
}		
%\vspace{-0.1in}
\end{table*}

==> tables/tab_hoi.tex <==

\begin{table}
\setlength{\tabcolsep}{5pt}
\footnotesize
\centering

%\resizebox{\textwidth}{!}{
% \begin{tabular}{
%     lccccccc
%     }

% \toprule
% & & \multicolumn{3}{c}{Default}  & \multicolumn{3}{c}{Known Obj} \\

% Model & Super
%     & \multicolumn{1}{c}{Full} & \multicolumn{1}{c}{Rare} & \multicolumn{1}{c}{NonR}
%     & \multicolumn{1}{c}{Full} & \multicolumn{1}{c}{Rare} & \multicolumn{1}{c}{NonR} \\

% \midrule
% \gpvtwo & 0-shot & - & - & - & - & - & -  \\
% Model A & Full & - & - & - & - & - & - \\
% Model B & Full & - & - & - & - & - & - \\
% \bottomrule
% \end{tabular}%}

 \begin{tabular}{
    lccc
    }

\toprule
& \multicolumn{3}{c}{Default}  \\

Model & \multicolumn{1}{c}{Full} & \multicolumn{1}{c}{Rare} & \multicolumn{1}{c}{NonR} \\

\midrule
\gpvtwo & 20.3 & 17.3& 21.2  \\

\bottomrule
\end{tabular}%}

% \vspace{-0.1in}
\caption{
\label{tab:hoi}
\textbf{Human Object Interaction.} \todo{compare to specialized?}}	
\end{table}


==> tables/table_concept_scaling_closed_word_full.tex <==


\begin{table*}
\setlength{\tabcolsep}{2pt}
\footnotesize
\centering

% \begin{subtable}[h]{1.0\textwidth}\centering
\resizebox{\textwidth}{!}{
\begin{tabular}{
    lc
    >{\columncolor{Color4}}c>{\columncolor{Color4}}c>{\columncolor{Color4}}c
    >{\columncolor{Color4b}}c>{\columncolor{Color4b}}c>{\columncolor{Color4b}}c
    >{\columncolor{Color4}}c>{\columncolor{Color4}}c>{\columncolor{Color4}}c
    >{\columncolor{Color4b}}c>{\columncolor{Color4b}}c>{\columncolor{Color4b}}c
    >{\columncolor{Color2}}c
    >{\columncolor{Color2b}}c>{\columncolor{Color2b}}c>{\columncolor{Color2b}}c>{\columncolor{Color2b}}c
    >{\columncolor{Color2}}c>{\columncolor{Color2b}}c
    >{\columncolor{Color3}}c>{\columncolor{Color3b}}c>{\columncolor{Color3}}c>{\columncolor{Color3b}}c
    }

\toprule
\multicolumn{2}{c}{} 
    & \multicolumn{12}{c}{\cellcolor{Color4}\cocosce}
    & \multicolumn{7}{c}{\cellcolor{Color2}\opensce}
    & \multicolumn{4}{c}{\cellcolor{Color3}\web} \\

\multicolumn{2}{c}{} 
    & \multicolumn{3}{c}{\cellcolor{Color4}\emph{VQA}}
    & \multicolumn{3}{c}{\cellcolor{Color4}\emph{Cap}} 
    & \multicolumn{3}{c}{\cellcolor{Color4}\emph{Loc}} 
    & \multicolumn{3}{c}{\cellcolor{Color4}\emph{Cls}}
    % & \multicolumn{3}{c}{\cellcolor{Color4}\emph{CiC}} \\
    & \multicolumn{1}{c}{\cellcolor{Color2}\emph{VQA}}
    & \multicolumn{4}{c}{\cellcolor{Color2}\emph{Cap}} 
    & \multicolumn{1}{c}{\cellcolor{Color2}\emph{Loc}} 
    & \multicolumn{1}{c}{\cellcolor{Color2}\emph{Cls}} 
    % & \multicolumn{1}{c}{\cellcolor{Color2}\emph{CiC}} 
    
    & \multicolumn{1}{c}{\cellcolor{Color3}\emph{All}} 
    & \multicolumn{1}{c}{\cellcolor{Color3}\emph{Noun}} 
    & \multicolumn{1}{c}{\cellcolor{Color3}\emph{Verb}} 
    & \multicolumn{1}{c}{\cellcolor{Color3}\emph{Adj}} \\

\multicolumn{1}{c}{Model} & \multicolumn{1}{c}{Web data} 
    & \cellcolor{Color4}\emph{Test} & \cellcolor{Color4}\emph{Sn} & \cellcolor{Color4}\emph{Unsn}
    & \cellcolor{Color4}\emph{Test} & \cellcolor{Color4}\emph{Sn} & \cellcolor{Color4}\emph{Unsn}
    & \cellcolor{Color4}\emph{Test} & \cellcolor{Color4}\emph{Sn} & \cellcolor{Color4}\emph{Unsn}
    & \cellcolor{Color4}\emph{Test} & \cellcolor{Color4}\emph{Sn} & \cellcolor{Color4}\emph{Unsn}
    % & \cellcolor{Color4}\emph{Test} & \cellcolor{Color4}\emph{Sn} & \cellcolor{Color4}\emph{Unsn} \\
    & \cellcolor{Color2}{} 
    & \cellcolor{Color2}\emph{In} & \cellcolor{Color2}\emph{Near} & \cellcolor{Color2}\emph{Out} & \cellcolor{Color2}\emph{All}
    & \cellcolor{Color2}{} & \cellcolor{Color2}{} 
    
    & \cellcolor{Color3}{} & \cellcolor{Color3}{} & \cellcolor{Color3}{} & \cellcolor{Color3}{}\\
    
\midrule
\gpvtwo & no web &  59.6 & 60.1 & 48.5 & 88.4 & 91.7 & 55.5 & 62.2 & \textbf{67.2} & 14.0 & \textbf{73.1} & 77.2 & \textbf{33.9} & \textbf{46.9} & 56.1 & 40.5 & 21.1 & 39.0 & 54.9 & 13.6 & 14.0 & 3.3 & 11.6 & 27.1 \\
\gpvtwo & with web & \textbf{59.9} & \textbf{60.3} & \textbf{49.7} & \textbf{89.2} & \textbf{92.1} & \textbf{58.0} & 62.2 & 67.0 & \textbf{14.8} & 73.0 & 77.2 & 32.6 & 46.8 & \textbf{60.8} & \textbf{47.0} & \textbf{33.4} & \textbf{46.3} & \textbf{58.7} & \textbf{26.5} & \textbf{47.0} & \textbf{25.1} & \textbf{43.0} & \textbf{73.0} \\
\bottomrule
\end{tabular}}


\caption{
\label{tab:concept_scaling_closed_world}
\textbf{Concept scaling using web data: Closed world experiment.} To eliminate the effect of VinVL features and \cc\ pretraining, we restrict \gpvtwo\ to \cocosce\ trained DETR features. Training jointly with \web\ still shows massive gains on \opensce\ and \web\ vs training with only \cocosce.
}		

\end{table*}

==> tables/web_detailed_stats.tex <==
\begin{table}[]
\footnotesize
    \centering
    \begin{tabular}{c|l}
        \toprule
        \textbf{} & \textbf{Statistics} \\
        \midrule
      \multirow{6}{*}{Concepts } &  Nouns: 10211 \\
      & Adjectives: 144 \\ 
      & Verbs: 298 \\
      & Noun-adjective pairs: 18616 \\
      & Noun-verb pairs: 9243 \\
      & \textbf{Total: 38072} (Nouns + Pairs) \\
      \midrule
      \multirow{4}{*}{Images} &  Noun images: 255073 \\
       & Noun-adjective images: 465146 \\
       & Noun-verb images: 230224\\
       & \textbf{Total: 950443} \\
       \midrule
      \multirow{5}{*}{QAs} & Templates: 26 \\
& Noun QAs: 1900886 \\
& Adjective QAs: 930292 \\
& Verb QAs: 460448 \\
& \textbf{Total: 3291626} \\
        \bottomrule
    \end{tabular}
    

    \caption{\textbf{Statistics about WEB10K}. \todo{Write caption}
    }
    \label{tab:webqa-templates}
\end{table}
\label{app:web-questions}


==> tables/web_stats.tex <==
% Please add the following required packages to your document preamble:
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{table*}[]
\small
\centering
\begin{tabular}{lcccl}
\toprule
\multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}Concept\\ Type\end{tabular}} & \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}Unique concepts\\ in Web data\end{tabular}} & \multicolumn{1}{c}{Queries} & \multicolumn{1}{c}{Sources}                          & \multicolumn{1}{c}{Question Types}                                                                      \\
\midrule
Noun                                                                       & 10213                                                                                     & 10213                       & \cite{Brysbaert2013Concreteness, Sharma18Conceptual}                                             & ``What object is this?''                                                                                \\
Adjective                                                                  & 148                                                                                       & 18616                       &  \cite{Sharma18Conceptual, Krishna17Visual, Farhadi2009DescribingOB, Lampert2009LearningTD, Kumar2009AttributeAS, Patterson2012SUNAD, Parikh2011RelativeA, Chen2012DescribingCB, Wang2013WeaklySL} & \begin{tabular}[c]{@{}l@{}}``What color is the object?''\\ ``What color is the armchair?''\end{tabular} \\
Verb                                                                       & 298                                                                                       & 9243                        & \cite{Yatskar2016SituationRV, ChaoHOIBench, Sharma18Conceptual,Liang2018VisualRD}                                & \begin{tabular}[c]{@{}l@{}}``What are they doing?''\\ ``What is the chef doing?''\end{tabular}          \\
\midrule
Total                                                                      & 10659                                                                                     & 38072                       &                                                      &                                                                                                        \\
\bottomrule

\end{tabular}
\caption{
\label{tab:web_stats}
\textbf{Statistics about \web~data collection}}
\end{table*}
